Scaling Up Deep Clustering Methods Beyond ImageNet-1K

Deep image clustering methods are typically evaluated on small-scale balanced classification datasets while feature-based $k$-means has been applied on proprietary billion-scale datasets. In this work, we explore the performance of feature-based deep clustering approaches on large-scale benchmarks whilst disentangling the impact of the following data-related factors: i) class imbalance, ii) class granularity, iii) easy-to-recognize classes, and iv) the ability to capture multiple classes. Consequently, we develop multiple new benchmarks based on ImageNet21K. Our experimental analysis reveals that feature-based $k$-means is often unfairly evaluated on balanced datasets. However, deep clustering methods outperform $k$-means across most large-scale benchmarks. Interestingly, $k$-means underperforms on easy-to-classify benchmarks by large margins. The performance gap, however, diminishes on the highest data regimes such as ImageNet21K. Finally, we find that non-primary cluster predictions capture meaningful classes (i.e. coarser classes).

==> checklist.tex <==

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\section*{Checklist}

% %%% BEGIN INSTRUCTIONS %%%
% The checklist follows the references.  Please
% read the checklist guidelines carefully for information on how to answer these
% questions.  For each question, change the default \answerTODO{} to \answerYes{},
% \answerNo{}, or \answerNA{}.  You are strongly encouraged to include a {\bf
% justification to your answer}, either by referencing the appropriate section of
% your paper or providing a brief inline description.  For example:
% \begin{itemize}
%   \item Did you include the license to the code and datasets? 
% \end{itemize}
% Please do not modify the questions and only use the provided macros for your
% answers.  Note that the Checklist section does not count towards the page
% limit.  In your paper, please delete this instructions block and only keep the
% Checklist section heading above along with the questions/answers below.
% %%% END INSTRUCTIONS %%%
We clarify that we include all the information related to the dataset and code in the appendix, which will be included as a separate file in the submission.
\begin{enumerate}

\item For all authors...
\begin{enumerate}
  \item Do the main claims made in the abstract and introduction accurately reflect the paper's contributions and scope? \answerYes{We did our best to encapsulate the most important findings in the abstract and introduction.}
  \item Did you describe the limitations of your work?
    \answerYes{Yes please see \Cref{sec:discussion} }
  \item Did you discuss any potential negative societal impacts of your work?
    \answerYes{We cannot identify any negative societal impacts in this work since we do not introduce a new dataset but focus on carefully creating new insightful benchmarks.}
  \item Have you read the ethics review guidelines and ensured that your paper conforms to them?
    \answerYes{All authors have read and are aware of the ethics review guidelines}
\end{enumerate}

\item If you are including theoretical results...
\begin{enumerate}
  \item Did you state the full set of assumptions of all theoretical results?
    \answerNA{Not applicable as we do not include any theoretical result in this work}
	\item Did you include complete proofs of all theoretical results?
      \answerNA{Not applicable as we do not include any theoretical result in this work}
\end{enumerate}

\item If you ran experiments (e.g. for benchmarks)...
\begin{enumerate}
  \item Did you include the code, data, and instructions needed to reproduce the main experimental results (either in the supplemental material or as a URL)?
   \answerYes{All the code with technical instructions, curated ImageNet21K-based benchmarks, and hyperparameters that reproduce our results are submitted as supplementary material and will be made publicly available upon acceptance.}
  \item Did you specify all the training details (e.g., data splits, hyperparameters, how they were chosen)?
     \answerYes{Yes, we did. Apart from the details and hyperparameters detailed in the appendix, we provide the data splits of the new benchmarks to enforce reproducibility.}
	\item Did you report error bars (e.g., with respect to the random seed after running experiments multiple times)?
    \answerYes{No, but we provide the standard deviations of our results in the supplementary material}
	\item Did you include the total amount of compute and the type of resources used (e.g., type of GPUs, internal cluster, or cloud provider)?
    \answerYes{Yes, we provide the hardware used to produce our results.}
\end{enumerate}

\item If you are using existing assets (e.g., code, data, models) or curating/releasing new assets...
\begin{enumerate}
  \item If your work uses existing assets, did you cite the creators?
  \answerYes{Yes, we have cited the creators of the dataset as well as all the follow-up works on which we based our analysis and new benchmarks.}
  \item Did you mention the license of the assets?
    \answerYes{Yes, in the appendix of the paper, we will report the individual licenses of all the datasets and benchmarks which we build upon.}
  \item Did you include any new assets either in the supplemental material or as a URL?
   \answerYes{Yes, the new asset is the image-label pairs, where some of the original labels have been reassessed as detailed in the main manuscript.}
  \item Did you discuss whether and how consent was obtained from people whose data you're using/curating?
    \answerNA{We believe this is not required in our case, to the best of our knowledge.}
  \item Did you discuss whether the data you are using/curating contains personally identifiable information or offensive content?
    \answerNA{To the best of our knowledge, ImageNet-1K and ImageNet21K do not include any identifiable information or offensive content according to the original publication. At the time of the submission, we are not aware of any offensive content.}
\end{enumerate}

\item If you used crowdsourcing or conducted research with human subjects...
\begin{enumerate}
  \item Did you include the full text of instructions given to participants and screenshots, if applicable?
     \answerNA{Not applicable to our work.}
  \item Did you describe any potential participant risks, with links to Institutional Review Board (IRB) approvals, if applicable?
    \answerNA{Not applicable to our work.}
  \item Did you include the estimated hourly wage paid to participants and the total amount spent on participant compensation?
     \answerNA{Not applicable to our work.}
\end{enumerate}

\end{enumerate}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%




==> tables/aaaaa.tex <==
\begin{table}
\centering
\begin{tabular}{l cccc}
\toprule
&   Top$1\rightarrow$1 & Top$1\rightarrow$L & Top$5\rightarrow$1 & Top$5\rightarrow$L  \\
\hline
\multicolumn{5}{l}{\textit{ImageNet21K using iBOT ViT-L}}  \\
$k$-means       & 23.38 & 26.55   & 39.92   & 46.17   \\
TEMI            & 23.74 & 27.05   & 42.66   & 48.84   \\
SCANv2          & 20.27 & 22.91   & 31.80   & 37.77   \\
  {Linear probing} &   {47.34} &  {51.26}   &  {76.36}   &  {79.76}  \\
\hline
\multicolumn{5}{l}{\textit{ImageNet1K-ReaL using MAE-R ViT-H}}  \\
 $k$-means      & 62.72 & 68.16   & 78.23   & 83.05          \\
 TEMI           & 66.40 & 73.07   & 82.03   & 86.74           \\ 
 SCANv2         & 69.79 & 75.89   & 84.63   & 89.37            \\
  {Linear probing} &  {81.13} & {88.19  }  &  {94.49  } &  {97.29  }\\
\bottomrule 
\end{tabular}
\end{table}

==> tables/sup_freq.tex <==
\begin{table}
    \centering
\begin{tabular}{l ccc}
\toprule
Dataset & \# samples & \# classes & Class frequency  \\
\midrule
Imbalanced  & 2.55M & 2113 & $[1035,1162]\mathrm{U}[1877,2997]$ &  & \\
Tiny       & 1.17M & 1060 &  $[1077,1139]$   \\
Small       & 3.46M & 3146 & $[979,1183]$     \\
Base        & 5.67M & 5230 & $[836,1239]$  \\
Large       & 7.79M & 7326 & $[661,1329]$ \\
Huge        & 9.88M & 9405 & $[514,1573]$  \\
\hline
ImageNet21K  & 11.06M & 10450 & $[451,2997] $     \\
\bottomrule
\end{tabular}
    \caption{Frequency-based ImageNet21K subsets with different degrees of imbalance.}\label{tab:freq-in21k-splits}
\end{table}


